Detection of Groups with Biased Representation in Ranking

Real-life tools for decision-making in many critical domains are based on ranking results. With the increasing awareness of algorithmic fairness, recent works have presented measures for fairness in ranking. Many of those definitions consider the representation of different ``protected groups'', in the top-$k$ ranked items, for any reasonable $k$. Given the protected groups, confirming algorithmic fairness is a simple task. However, the groups' definitions may be unknown in advance. In this paper, we study the problem of detecting groups with biased representation in the top-$k$ ranked items, eliminating the need to pre-define protected groups. The number of such groups possible can be exponential, making the problem hard. We propose efficient search algorithms for two different fairness measures: global representation bounds, and proportional representation. Then we propose a method to explain the bias in the representations of groups utilizing the notion of Shapley values. We conclude with an experimental study, showing the scalability of our approach and demonstrating the usefulness of the proposed algorithms.

==> response.tex <==
\twocolumn


\section*{Revision Summary}

We thank the reviewers for their close reading and constructive comments, which have helped us improve the paper and guided us in revising it. For convenience, the main changes are colored in \rev{green} in the revised manuscript. We clarified the problem setting and motivation, elaborated on the experimental setting, and better positioned our work with respect to related works. Due to space constraints, the proofs are deferred to~\cite{full}.
% \yuval{Something about the main changes: clarifying the problem setting and positioning with respect to related work}
\subsection*{Reviewer 1}
\paragraph*{Comment O1} Problem formulation: The problem motivates the search for patterns, as the user may not know what patterns to search for. However, it still relies on a number of parameters that may be harder to justify. Please discuss the real-world implications of choosing k, $L_k$, $U_k$, and other parameters.

Additionally, the search space of patterns is not relative to all data points in the dataset. It is very likely that no mechanism can generate a fair ranking (because the dataset does not contain enough representation from certain groups). I think the definition of representation should be relative to the number of times that pattern exists in the dataset.

\paragraph*{Revision}\rev{
We agree with the reviewer that there are many ways to think about fairness, and one way may be more appropriate than another in any specific situation. This is precisely why we try not to define one specific concept of fairness in our paper. Instead, we harness fairness measures from the literature on ranking algorithms. In particular, we support two prominent classes of fairness measures. The first, built on the fundamental definition presented in~\cite{CelisSV18}, restricts the representation of groups using upper and lower bounds. The second definition relies on a recent line of works considering proportional representation where the representation of each group should be proportional to its size in the data (i.e., relative to the number of times that pattern exists in the dataset). While the proportional representation gives the user an intuitive definition, the definition of global representation allows the user to actively control the bounds over the representation of different groups in the top-$k$ ranked items, even if their representation in the overall data is low/high.

For instance, consider a ranking algorithm for job applicants in fields that are dominated by men (e.g., tech companies). If the company wishes to increase the representation of women they hire but their application number is low and only the top-$k$ ranked applicants are invited for an interview, by using proportional representation, their number in the top-$k$, and as a result, the number of women invited to an interview, would be low as well. The fundamental definition of~\cite{CelisSV18} allows the user to define bounds over the representation of the protected groups in the data for different values of $k$. Following this definition, we defined the global bounds representation problem, which assumes no prior information regarding the identity of the protected groups and aims to identify \emph{all} groups with biased representation. Note that our goal is to report \emph{only} the most general patterns (groups), providing a concise description of these groups. The definition of~\cite{CelisSV18} indeed requires a relatively high number of parameters however it allows the user manually control the representation of different groups. Note that in our case, the number of parameters is lower as the bounds are defined globally and not per group. We included a discussion after Problem~\ref{problem:ranking:proportional}.}


% \begin{itemize}
%     \item Rewrite/rephrase the relevant text and explain the rationale (based on the definition of~\cite{CelisSV18}), allows users to maintain an adequate representation of minorities in the top-$k$ even if they are not well represented in the overall data.
%     \item We consider relative representation as well (problem~\ref{problem:ranking:proportional}), this is indeed a natural definition.
%     It makes sure all groups have a representation proportional to their overall sizes in the data.
% \end{itemize}
% }
% \yuval{Maybe he meant relative instead of absolute values?}
\paragraph*{Comment O2} Please explain the motivation to vary $k$. It is unclear why a user may want to consider multiple different values of $k$ and how they should be set. On fixing $k$, wouldn't it become the same problem as that of fairness testing? Please discuss the differences and implications of this generalization.

\paragraph*{Revision}\rev{ Thank you for this important comment.
 Fairness definitions for ranking typically account for the order of tuples in the output (or the top-$k$ tuples), i.e., it is not enough to have adequate representation in the top-$k$, every prefix of the output should be ``fair'' as well.
 Intuitively, accounting for a range of $k$'s ensures that the ranking is fair for any \emph{position} in the ranking. For instance, if the top-$10$ items consist of $5$ students with an urban address and $5$ students with a rural address, but the students with urban addresses are in the $1$-$5$ positions of the ranking, the output may seem ``fair'' if we are only interested in selecting the top-$10$ students, but if the positions within the top-$10$ are also important (e.g., position in the ranking affects an award amount), then clearly this ranking is unfair. We now explain this at the beginning of Section~\ref{sec:problem}.

 In fairness testing, the protected groups are assumed to be known in advance. Even for a fixed $k$ value, the problem would be to identify groups with biased representation in the top-$k$ ranked items for the given $k$ with no prior knowledge of the protected groups. In this case, however, the problem (in the case of global bounds) becomes somewhat similar to the problem of identifying groups with insufficient representation studied in~\cite{AsudehJJ19}. The algorithm presented in~\cite{AsudehJJ19} is indeed used in our baseline solution. We note that~\cite{AsudehJJ19} does not consider the problem of proportional representation of groups.
}


\paragraph*{Comment O3} Experiments: Please add a discussion of how parameters were chosen, how continuous attributes were bucketized and its impact on the experiment results. I expect that the running time grows exponentially with their domain.

\paragraph*{Revision}
\rev{
Multiple parameters affect the algorithms' running time and output, and in the experimental evaluation, we examine their effect. Following the goals of fairness in ranking (ensuring fairness for any position), we set gradually increasing bounds on group representation in the top-$k$ ranked items as $k$ increases. Since we aim at reporting the detected groups to the user, we set the parameters such that the number of reported groups in most cases is between $1$ to $100$. This way, the reported results reflect the algorithm's performance under expected typical usage scenarios. We experimentally evaluated the algorithms using different parameter settings and observed similar trends.

A major factor in the algorithm's running time is the search space it traverses to find the groups with biased representation. The size of the search space is determined by multiple input parameters: the size of the pattern graph, the threshold over the size of reported groups, and the representation bounds. The size of the pattern graph is a function of the number of possible patterns, i.e., the number of attributes $\mathcal{A}$ and the active domain size of each attribute $|Dom(A_i)|$ for each $A_i\in\mathcal{A}$. Concretely, the pattern graph size is $\prod_{i=1}^{|\mathcal{A}|}(|Dom(A_i)|+1$ (see~\cite{AsudehJJ19} for the analysis).
The bucketization indeed affects the size of the active domain and, as a result, the size of the pattern graph. Moreover, it affects the possible group definitions and their representation in the top-$k$, which can also affect the running time. 
The following figure shows an example of the effect of bucketization on the running time of the algorithms. We bucketized \texttt{absence} attribute (with values 0-93) of the Student dataset into a different number of bins and report the running times.

\begin{center}
\includegraphics[width = 0.8\linewidth]{ExperimentFigures/binning_time_prop_student_26att.png}
\end{center}
The general trend is indeed an increase in the running time, but we also observed cases where the running time decreases when the number of bins increases.
The bucketization of categorical values and their effect on the output is an intriguing direction for future work.
This work assumes that the attribute values used for group definitions are categorical. For the experiments, we equally bucketized continuous attributes, e.g., age, into 3-4 bins, based on their domain and values. 
% In the student dataset, grades are buketized into $4$ and other numeric values onto 3 bins. The German dataset consists of 3 numerical attributes: for DurationMonth and ages we used 3 bins, and for the CreditAmount we used 4 bins. The numerical attributes in the COMPAS dataset were preprocessed similarly to~\cite{AsudehJJ19} 
%so that these attributes divide the data into different groups minimizing the effect on the running. 
We added a discussion in the parameters setting paragraph in Section~\ref{sec:exp}.}

% The running time of the algorithms may be affected by multiple parameters. The
% We experimentally evaluated the algorithms using different parameters setting
% }

\paragraph*{Comment O4} Theorem 3.3 shows hardness but also exposes that the proposed problem statement may not be sufficient to help an end user. How can someone review an exponential number of patterns?

\paragraph*{Revision}\rev{
Thank you for raising this important point. While the theoretical analysis shows that the number of patterns may be exponential, in practice, their number is significantly lower, allowing reasonable running times for our algorithms. For example, in our experimental evaluations, in $97.58\%$ of the times, the number of the reported groups was less than $100$ patterns, and in $51.13\%$ of the times, it was less than $25$ patterns. Even for a large number of attributes of $33$ (in the Students dataset), the maximal reported group number was $225$.

We agree that presenting many results (even $200$ patterns) may overwhelm the user. We note that the output may be organized by $k$ value and ranked by the groups' overall size in the data or by the bias in their representation (the difference between the required representation and the actual representation). We address this point at the end of Section~\ref{sec:problem}. 


% \begin{itemize}
%     \item Show that this is typically not the case -- report the number of identified groups in the experiments? \jinyang{Many of them has a large output actually... because we use the same set of parameters that may work only for a few situations in all experiments}
%     \item Order them by size/representation bias? \jinyang{Order by size, or define representation bias = $|U_k - s_{R^k(D)}(p)|$ for global bounds, and bias  = $|\frac{s_{R^k(D)}(p)}{k} - \alpha \frac{s_{D}(p)}{|D|}|$}
% \end{itemize}
}

% \paragraph*{Revision}\rev{
% \begin{itemize}
%     \item Show that this is typically not the case -- report the number of identified groups in the experiments? \jinyang{Many of them has a large output actually... because we use the same set of parameters that may work only for a few situations in all experiments}
%     \item Order them by size/representation bias? \jinyang{Order by size, or define representation bias = $|U_k - s_{R^k(D)}(p)|$ for global bounds, and bias  = $|\frac{s_{R^k(D)}(p)}{k} - \alpha \frac{s_{D}(p)}{|D|}|$}
% \end{itemize}
% }



\subsection*{Reviewer 2}

\paragraph*{Comment O1} Last paragraph of the related work: mentions a difference between the pattern graph and the powerset lattice used in frequent itemset mining and FD discovery. It might be useful to compare to CFDs (conditional functional dependencies) as well since they include patterns.

\paragraph*{Revision} \rev{Thank you for this comment! We added a discussion on CFDs at the end of the Related work section. Some algorithms for discovering CFDs indeed resembles the top-down search as they also consider patterns and lattice of patterns. However, the difference in the end goal (discovering CFDs versus identifying groups with biased representation) leads to differences in the pruning techniques in the top-down search.}

\paragraph*{Comment O2} At the end of section 6, there is a comparison to previous work [24] (\rev{\cite{pastor2021identifying} in the revised paper}). In the last paragraph, it would be good to clarify why the proposed solution was more effective than [24]. This might be hard to do without a user study or expert feedback, but it would be nice to say something about the utility or importance of the discovered groups. In other words, why is [24] insufficient in practice?

\paragraph*{Revision}
\rev{Thank you for the comment. We clarify the differences by adding the following at the end of the comparison (at the end of Section~\ref{sec:exp}).

The key difference between our algorithms and the solution of~\cite{pastor2021identifying} lies in the definitions of the groups they aim to identify. The two solutions deal with a similar problem, however, our solution prefers concise groups (most general pattern) while the solution of~\cite{pastor2021identifying} is designed to identify \emph{all} groups with sufficient representation in the overall data and high divergence (a measure of ``unfairness''). As a result, the output of~\cite{pastor2021identifying} is typically larger and contains subgroups that are consumed by each other. Finally, the work of~\cite{pastor2021identifying} considers a single $k$ while we consider a range of $k$'s, aligning with fairness definitions in the literature, making the solution fair for any position in the top-$k$.}

% while our solutions prefer concise groups (most general pattern).

% the main difference between our solution and~\cite{pastor2021identifying} is the definition of the groups the algorithm should report. Our solution prefers concise groups (most general pattern) while the solution of~\cite{pastor2021identifying} reports \emph{all} the groups with sufficient representation in the overall data and high divergence (a measure of ``unfairness''). As a result, the output of~\cite{pastor2021identifying} is typically larger. Moreover, the solution ~\cite{pastor2021identifying} ranks the reported groups by their divergence and, as a result, may report subgroups that are consumed by each other. Finally, the work of~\cite{pastor2021identifying} considers a single $k$ while we consider a range of $k$'s, aligning with fairness definitions in the literature, making the solution fair for any position in the top-$k$.}

\paragraph*{Additional remark} Related work: there is a sentence that should be split into two sentences: "In contrast, our solution considers all attributes as possible explanations this requires an additional aggregation step in the computation of the Shapley values."

\paragraph*{Revision} \rev{Thank you! Fixed.}
